Hyperbolic Attention Networks

We introduce hyperbolic attention networks to endow neural networks with enough capacity to match the complexity of data with hierarchical and power-law structure. A few recent approaches have successfully demonstrated the benefits of imposing hyperbolic geometry on the parameters of shallow networks. We extend this line of work by imposing hyperbolic geometry on the activations of neural networks. This allows us to exploit hyperbolic geometry to reason about embeddings produced by deep networks. We achieve this by re-expressing the ubiquitous mechanism of soft attention in terms of operations defined for hyperboloid and Klein models. Our method shows improvements in terms of generalization on neural machine translation, learning on graphs and visual question answering tasks while keeping the neural representations compact.

==> 130-hyperbolic-relation-networks.tex <==
\section{Hyperbolic Relation Networks (HRN)}

Relation Networks (RNs)~\cite{santoro2017simple} are a neural network architecture designed for reasoning about the relationships between objects.  A Relation Network operates on a set of object $O$ by applying a shared operator to each pair of objects $\left(o_i,~o_j\right) \in O\times O$.  Each pair is augmented by some global information, and the result of each relational operation is passed through a further global transformation.

The general Relation Network can be written as \todo{Picture of a relation net}
\begin{align}
    RN(O, q) = f\left(\sum_{ij}g(o_i, o_j, q)\right)
\end{align}
where $f$ is the global transformation, $g$ is the relational transformation, and $q$ is an additional global input.  We augment the RN architecture by introducing weights on the interaction terms
\begin{align}
    RN(O, q) = f\left(\sum_{ij}\alpha_{ij}g(o_i, o_j, q)\right)
\end{align}
and we interpret the resulting architecture as performing an attentive read operation over the relation representations produced by $g$.  Interpreting the operation in this way allows us to (1) compute the attention weights by comparing hyperbolic distances between relations and (2) replace the weighted average with the hyperbolic midpoint operation from Equation~\ref{eq:gyromidpoint}.  This leads to a model where
\begin{align}
    \alpha_{ij} &= \operatorname{sigmoid}(-\beta d(\operatorname{concat}(o_i, q), \operatorname{concat}(o_j, q)) - c) \\
    \vg_{ij} &= g(o_i, o_j, q) \\
    HRN(O, q) &=  f\left(\sum_{ij}\left[\frac{\alpha_{ij}\gamma_{\vg_{ij}}}{\sum_{uv} \alpha_{uv}\gamma_{\vg_{uv}}}\right]\vg_{ij}\right)
\end{align}
Interpreting the Relation Network as learned message passing on a graph over objects, the attention weights take on the semantics of edge weights, where $\alpha_{ij}$ can be thought of as the probability of the the (directed) edge $o_j \to o_i$ appearing in the underlying reasoning graph.  Using the hyperbolic distance between object representations to set this probability amounts to assuming a power-law prior on the degree distribution of the reasoning graph. \md{Connect this to the discussion of inductive bias of hyperbolic space.}


==> 140-hyperbolic-transformer.tex <==
\section{Hyperbolic Transformer (HT)}
\todo{Clean up this part}
In our take on transformer model, we basically focus on modifying the way attention works on the transformer model from Google Brain \citep{vaswani2017attention}. (These guys mention on page 9 that they think more sophisticated matching functions than dot product may help).

The original transformer model defines the attention in the following way:

The attention function is described as mapping a query and a set of key-value pairs to an output, where the query, keys, values, and output are all vectors.  The output is computed as a weighted sum of the values, where the weight assigned to each value is computed by a compatibility function of the query with the corresponding key.

\subsection{Scaled dot product attention}
\label{sec:scaled-dot-prod}

The core operation in the transformer model is their scaled dot-product attention operation, which is an attentive read operation with
\begin{align}
    f(\vq,\vk) = \frac{1}{\sqrt{d}}\left<\vq,\vk\right>
\end{align}
where $d$ is the dimensionality of $\vq$ and $\vk_i$.  We replace this method of computing weights with a hyperbolic matching function
\begin{align}
    f(\vq, \vk) = -\beta d(\vq, \vk) - c
\end{align}
where the additional bias term is added because distances are non-negative, as discussed in Section~\ref{sec:hyper-attention-weights}.  We also use the Einstein midpoint to combine the retrieved values, leading to a fully hyperbolic attentive read operation.  The full transformer model applies attention many times, with each read head in each layer performing an attentive read for each element of the sequence being processed.  We preserve this structure, and although we have written the matching function here for a single key-value pair, it is straightforward to produce an efficient vectorized implementation to perform many hyperbolic attentive reads in parallel.

The original transformer paper considers only softmax attention \citep{vaswani2017attention}, but we experiment with both softmax and sigmoid operations for computing the attention weights in our hyperbolic models.
\mati{we should mention why we use sigmoids. At least for visual questin answering this should make sense as sigmoids don't penalize two parts of the image so strongly if both are relevant while softmax does}

\subsection{Hyperbolic Recursive Transformers (HRT)}
\alert{Discuss about the hyperbolic recursive transformers in this subsection which we use for the Graph Problems. --CG}
See Figure \ref{fig:RecursiveHyperbolicTransformer}.

\begin{figure}
\begin{minipage}[c]{0.5\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{HyperboloidAttention_v2.pdf}
    \caption{Hyperbolic self-attention mechanism.}
    \label{fig:HyperbolicAttention}
\end{minipage}
\hfill
\begin{minipage}[c]{0.42\linewidth}
    \includegraphics[width=0.9\linewidth]{HyperboloidTransformer.pdf}
    \caption{Hyperbolic recursive transformer (HRT) model.}
    \label{fig:RecursiveHyperbolicTransformer}
\end{minipage}%
\end{figure}
